Wild Patterns Reloaded: A Survey of Machine Learning Security against Training Data Poisoning

The success of machine learning is fueled by the increasing availability of computing power and large training datasets. The training data is used to learn new models or update existing ones, assuming that it is sufficiently representative of the data that will be encountered at test time. This assumption is challenged by the threat of poisoning, an attack that manipulates the training data to compromise the model's performance at test time. Although poisoning has been acknowledged as a relevant threat in industry applications, and a variety of different attacks and defenses have been proposed so far, a complete systematization and critical review of the field is still missing. In this survey, we provide a comprehensive systematization of poisoning attacks and defenses in machine learning, reviewing more than 100 papers published in the field in the last 15 years. We start by categorizing the current threat models and attacks, and then organize existing defenses accordingly. While we focus mostly on computer-vision applications, we argue that our systematization also encompasses state-of-the-art attacks and defenses for other data modalities. Finally, we discuss existing resources for research in poisoning, and shed light on the current limitations and open research questions in this research field.

==> sections/other_attacks_defenses.tex <==
\subsection{Other Attacks}
We considered so far data poisoning attacks in the context of  classification for the vision domain. In the following, we give a short overview of existing attacks  in other application domains, and  for other learning paradigms such as unsupervised learning and reinforcement learning.

\subsubsection{Other Application Domains}
%We start with the application are of security, where the study of poisoning originated. We then review video, audio and graph classification as well as federated learning and regression. 
~\newline\myparagraph{Security.} 
The first work on training-time attacks in security, by \citet{kearns93learningmalicious}, was a theoretical analysis of Probably Approximately Correct (PAC) models. Real world attacks were later studied on worm signature classifiers~\citet{perdisciWormSignature2006} and spam classifiers~\citet{nelson08spam}, respectively encompassing availability and targeted poisoning. %An actual attack on a worm signature classifier was introduced by \citet{perdisciWormSignature2006}, where the adversary pollutes the dataset to mislead the signature extraction algorithms.
%To this end, the adversary pollutes the dataset with suspicious flows created by using fake invariant sub-strings that mislead the signature extraction algorithms.
%Furthermore, \citet{nelson08spam} studied poisoning against spam classifiers based. They assume the attacker sends malicious emails containing many words likely to occur in legitimate emails, and the victim will use them for training/updating the spam filter system (SpamBayes). In this way, legitimate emails are likely to be classified as spam since they contain words used in the adversary's generated spam emails.
More recently, \citet{severi_explanation-guided_2021} leveraged explainable machine learning techniques to backdoor malware classifiers, preserving the binary's functionalities. %The challenge here was to design a backdoor trigger capable to preserve binary's functionalities.
\myparagraph{Video.}
%Similar challenges are faced when targeting video classification.
%For example \citet{zhao_clean_video_2020} observed that image-based backdoor attacks (such as \citet{turner_clean-label}) can fail when targeting video recognition models, due to the general higher data dimensionality and sparsity on the training dataset. To this end, they enhance the attack effectiveness by injecting a cleverly optimized universal adversarial trigger in each frame of the video.
\citet{zhao_clean_video_2020} observed that image-based backdoor attacks (such as \citet{turner_clean-label}) can fail when targeting video recognition models, due to the general higher data dimensionality and sparsity on the training dataset. To this end, they enhance the attack effectiveness by injecting a cleverly optimized patch trigger in each frame of the video. %universal adversarial trigger in each frame of the video. 
\myparagraph{Audio.} 
\citet{venomave_aghakhani_2020} extended the work in \cite{aghakhani20bullseye} to generate poisoning samples against automatic speech recognition models so that the system mis-recognizes each frame of the target audio file. For backdoor poisoning attacks, the trigger is defined as a special audio track \citep{liu_trojaning_2018,Xu2021MetaAudio,Koffas2021Ultrasonic}, possibly inaudible to not raise human suspicion~\cite{Koffas2021Ultrasonic}. 
\myparagraph{NLP.} NLP models introduce a dependency between inputs, giving importance to the order of sentences, and small variations may change the inputs' semantics. The first challenge is considered by \citet{liu_trojaning_2018} and \citet{badnl_chen_2020}, where the adversary arbitrary manipulates the text, but at a fixed position.  \citet{trojaning_nlp_zhang_2020} enhanced the attack stealthiness by using natural sentences as triggers that ensure the fluency and context-awareness of the sentences. 
\myparagraph{Graphs.} When dealing with graph data the adversary has to search for edges or nodes perturbation that optimize the attacker's goal. %: sabotaging the classification model. 
\citet{Liu19GraphSSL}, \citet{Zugner19GraphSSL}, and  \citet{BojchevskiG19NodeEmbedding} showed that small graph perturbations compromise the performance or integrity of cutting-edge graph neural networks. Regarding backdoor poisoning, random \cite{Zhang21FixedBackdoorGraph} or topological preserving \cite{Xi21GraphBackdoor} subgraphs are used as triggers to mount the attack.
% federated learning
\myparagraph{Federated Learning.}
In federated learning applications, each client has their own data and model, and shares with a central server only the resulting model or gradient updates, but not the local data~\cite{Tolpegin20federflip}. 
Existing works showed how an attacker, controlling a few clients, can alter local data to share poisoning models or updates with the server, with the side effect of compromising the overall performance of the server's model \cite{Tolpegin20federflip, Cao19FederFlip,Zhang19GanFeder}.
Similarly, \cite{Bagdasaryan20BackdoorFeder,Bhagoji19BackdoorFeder, Sun19BackdoorFeder,Xie20DBA} implant the trigger in the client's model, so that also the server's model will be influenced in incorporating the backdoor. 

\myparagraph{Regression Learning.} Regression models are supervised learning approaches that predict a numerical response variable, instead of a categorical label. Existing approaches for poisoning regression are similar to classification and rely on solving bilevel optimization problems~\cite{feng2014regression, Liu2017RobustLR, jagielski2018manipulating, muller2020regression}. 

\subsubsection{Other Learning Paradigms}
We now review poisoning attacks in other learning paradigms such as unsupervised learning and reinforcement learning.

\myparagraph{Unsupervised Learning.}
Poisoning in unsupervised learning has been first investigated by \citet{rubinstein2009antidote} and \citet{kloft2010anomaly}, where indiscriminate poisoning attacks have been proposed to mislead anomaly detection systems. Instead, \citet{Biggio2013IsDC}, \citet{cina2022clustering}, and \citet{Biggio2014PoisoningBM} showed that even clustering algorithms are vulnerable in the presence of malicious noise. A crucial challenge for the attacker is that the optimization of the attack has to face with non-differentiable algorithms (\ie, K-means), thus limiting the application of existing gradient-based algorithms. 
\myparagraph{Reinforcement Learning.}
Last but not least, significant work has also been done in the field of reinforcement learning. Whereas few poisoning attacks in reinforcement learning attempt to reduce overall accuracy~\cite{kiourti2020trojdrl}, most attempt to teach the agent predefined behavior by changing the rewards and the environment~\cite{behzadan2017vulnerability} or the rewards~\cite{zhang2020adaptive,huang2019deceptive,rakhsha2020policy,wang2020reinforcement}.
%Backdoor poisoning in reinforcement learning boils down to one or several specific actions that are induced when the victim agent is confronted with a predefined setting, which corresponds to the trigger in the vision domain. The performance on an unchanged or clean environment should not be affected by the trigger. Such a trigger can be implanted by either altering the environment \cite{xu2021transferable,wang2021backdoorl,ashcraft2021poisoning}, the rewards~\cite{ma2018data} or the learner's observations~\cite{foley2022execute}.
Backdoor poisoning in reinforcement learning boils down to one or several specific actions that are induced when the victim agent is confronted with a triggering setting. Such a trigger can be implanted by either altering the environment \cite{xu2021transferable,wang2021backdoorl,ashcraft2021poisoning}, the rewards~\cite{ma2018data} or the learner's observations~\cite{foley2022execute}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Other Defenses}
In contrast to attacks  with application-specific triggers, defenses can be more generic. Some defenses are evaluated on domains as diverse as spam and vision data~\cite{liu2018fine,paudice2018label}, or classification and regression~\cite{diakonikolas2019sever}. Below, we give a short overview on state of the art of defenses in other domains than vision and other learning paradigms than classification. 
%We start with defenses for security applications, as these were historically developed first. We then continue with audio classification, natural language processing (NLP), graph classification, and federated learning. We then tackle regression, unsupervised learning, and reinforcement learning.
%Approaches that have been discussed in detail above will be briefly mention if they are applicable to  specific applications. 

\myparagraph{Other Application Domains.}
In the area of security, defenses against indiscriminate poisoning attacks can be split in robust training on spam~\cite{diakonikolas2019sever,biggio2011bagging} or intrusion detection~\cite{biggio2011bagging,nelson2009misleading}, and training data sanitization on spam~\cite{frederickson2018attack,paudice2018label} or malware classification~\cite{taheri2020defending}.
%2. video
In the video domain, \citet{zhao_clean_video_2020} show that data augmentation,  Neural Cleanse~\cite{wangneural}, and Spectral Signatures~\cite{tran2018spectral} can be used to defend against backdoors.
%3. audio
The only backdoor defense on audio data is a model sanitization approach based on fine-tuning~\cite{liu2018fine}. %, which is also evaluated on vision data.
%4. nlp
In NLP, one backdoor defense relies on a perplexity score to sanitize test data~\cite{qi2020onion}, a second implements an importance score for training data sanitization~\cite{chen2020mitigating}.
%test data sanitization, training data sanitization
%5. graphs DONE
\citet{tang2020transferring} mitigate indiscriminate poisoning on graph neural networks with a method similar to adversarial training. A second approach combines Bayesian uncertainty and distillation~\cite{shanthamallu2021uncertainty}. Both defenses thus implement robust training.

%6. federated learning
%Most defenses were proposed in the context of federated learning. 
To mitigate label-flip attacks in federated learning, robust training can be implemented using game theory~\cite{zhang2017game} or
pivotal learning~\cite{zhang2020defending}.
In the same setting, training data can be sanitized using 
%The training data of the federated learning can further be sanitized from poisonous points using 
outlier detection among the users~\cite{hayes2018contamination} or by training on  subsets which yield good accuracy~\cite{zhao2019pdgan}.
%7. regression
To protect regression from indiscriminate poisoning, robust training based on robust optimization~\cite{jagielski2018manipulating,diakonikolas2019sever} or robust subset training~\cite{wen2021great} have been proposed.

\myparagraph{Beyond Supervised Learning.}
In unsupervised learning, indiscriminate poisoning defenses for anomaly sensors are based on micro-models~\cite{Cretu2008Casting-out-Dem} trained on subsets of the data, thus implementing both robust training and training data sanitization. Pure robust training instead uses robust statistics, for example the median instead of the mean~\cite{rubinstein2009antidote}.
%propose a more robust variant of PCA that incorporates outlier resistant statistics like the median instead of the mean. While the latter falls into the category of robust training, the first approach lies between the categories of robust training and training data sanitization.
%Both DoS and backdoor poisoning have been studied in the area of reinforcement learning. Most 
Indiscriminate poisoning defenses in reinforcement learning are robust training approaches, and use minmax optimization~\cite{banihashem2021defense}, data augmentation~\cite{wang2020reinforcement} or specific reward heuristics that increase the cost of poisoning the agent~\cite{everitt2017reinforcement}. %propose 
For label flip attacks, data sanitization for reinforcement learning model the attacker explicitly and then re-flip identified labels~\cite{han2020adversarial}.
  Finally, \citet{wang2021backdoorl} find that model sanitization using fine-tuning is of limited success for reinforcement learning.

\myparagraph{Conclusion.} Most defenses are designed for the computer vision domain, and it is not always clear if and how to adapt them to other settings. 
Several papers showed how to transfer insights from vision defenses to protect against poisoning attacks in video applications and reinforcement  learning~\cite{zhao_clean_video_2020,wang2021backdoorl}. 
The large majority of surveyed defenses outside vision are applicable to indiscriminate poisoning and most of them operate during training, leaving many open questions about developing test-time defenses and backdoor defenses in various application domains.  


==> sections/timeline.tex <==
\begin{comment}
\begin{figure}
\centering
    \vspace{-1.5cm}
    \resizebox{\columnwidth}{!}{\input{timeline/timelinev2/tlall.tex}}
    \vspace{-2.5cm}
    \caption{Timeline One Page}
    \label{fig:TLbd}
\end{figure}
\end{comment}

\begin{figure}
\centering
    \vspace{1cm}
    \resizebox{\columnwidth}{!}{\input{timeline/timelinev3/tlall.tex}}
    \vspace{-2.5cm}
    \caption{Timeline One Page}
    \label{fig:TLbd}
\end{figure}


==> tables/defenceAttackTable.tex <==
\begin{comment}
\begin{table}[]
\centering
\caption{Matching poisoning test time attack strategies and defenses applied after training. For each defense, we denote on which type of attack strategies the defense was evaluated. We omit indiscriminate attacks, as there are no corresponding defenses at test time (yet). }\label{table:testDefenses}
\resizebox{\textwidth}{!} {%
\begin{tabular}{lcm{2.1cm}>{\raggedright}m{2.35cm}>{\raggedright}m{2.5cm}m{2.5cm}}
\toprule
\multicolumn{2}{c}{Attack}  & \multicolumn{4}{c}{Defenses} \\
\cmidrule(r){1-2}\cmidrule(r){3-6}

 & Strategy  &
 Model \newline  inspection &
  Trigger \newline  reconstruction &
  Model \newline  sanitization &
 Test data \newline  sanitization \\
 \midrule


\multirow{3}{*}{Backdoor}&
  Trigger(P) &
  \cite{tang2019demon,chen2018detecting,kolouri2020universal,zhang2021tad,shen2021backdoor,chen2019deepinspect,Xu2021MetaAudio,bajcsy2021baseline,xiang2021red,soremekun2020exposing} &
  \cite{guo2019tabor,wangneural,liu2019abs,udeshi2019model,qiao2019defending,cheng2020defending,dong2021black,xiang2021reverse} &
  \cite{liu2018fine,zeng2020deepsweep,yoshida2020disabling,li2021neural,zhao2020bridging,qiao2019defending,chen2019deepinspect,zhu2020gangsweep,wu2021adversarial} &
  \cite{doan2020februus,li2020rethinking,zeng2020deepsweep,veldanda2020nnoculation,wangneural,chou2018sentinet,gao2019strip,sarkar2020backdoor,qi2020onion,villarreal2020confoc} \\
  
  %\addlinespace
& Trigger(F) &
  \cite{tang2019demon,shen2021backdoor,huang2019neuroninspect,Xu2021MetaAudio,soremekun2020exposing} &
  \cite{xiang2020detection,zhu2020gangsweep,liu2019abs,xiang2021red} &
  \cite{zhu2020gangsweep, zeng2020deepsweep,li2021neural,wu2021adversarial} &
  \cite{zeng2020deepsweep} \\
  
  %\addlinespace
& Trigger(S) & & & \cite{DBLP:conf/iccd/LiuXS17} &
  \cite{DBLP:conf/iccd/LiuXS17} \\
  
  %\addlinespace
  
Targeted &  - & \cite{zhu2021clear} & & \cite{zhu2021clear} & \\

  \bottomrule
\end{tabular}}
\end{table}
\end{comment}




==> tables/testmatch.tex <==
\begin{comment}


\begin{table}[t!]
\centering
\caption{Matching poisoning training time attack strategies and training time defenses. For each defense, we depict on which attack strategy (as defined in Section~\ref{sec::attacks}) the defense was evaluated. We omit strategies in the table that were not mitigated yet, including clean label optimized bilevel indiscriminate (BL), and backdoors with a semantical (T$^S$) trigger, optimized bilevel backdoors (BL) and clean label feature collision backdoors (FC). Finally, \emph{in theory} defenses working on targeted optimized attacks (BL, FC) might also mitigate the same class of backdoor optimized attacks and vice versa.}\label{table:trainDefenses}
%\resizebox{\textwidth}{!} {%
\begin{tabular}{cccrr}
\toprule
\multicolumn{2}{c}{Attack} & \multicolumn{3}{c}{Defenses} \\
 \cmidrule(r){1-3}\cmidrule(r){4-5}
 &Strategy & Clean label& Training data sanitization & Robust training \\
\midrule
\multirow{2}{*}{Indiscriminate} 
& LF & &\cite{paudice2018label, DBLP:journals/corr/LaishramP16,taheri2020defending} &
  \cite{hong2020effectiveness,levine2020deep,biggio11labelnoise,DBLP:conf/itasec/DemontisBFGR17,rosenfeld2020certified}\\
& BL & & \cite{frederickson2018attack,2017arXiv170603691S} & \cite{nelson2009misleading,biggio2011bagging, jia2020certified, private_learners_ma_2019} \\
%& BL & \checkmark & & \\
  \addlinespace 
\multirow{3}{*}{Targeted}  
&  BL & & \cite{frederickson2018attack,hayase2021spectre} & \\
& FC & \checkmark & \cite{peri2020deep} & \cite{geiping2021doesn,borgnia2021dp,li2021anti,hong2020effectiveness}\\
& BL & \checkmark & & \cite{geiping2021doesn,borgnia2021dp,borgnia2021strong}\\
\addlinespace
\multirow{3}{*}{Backdoor}
& T$^P$ &  & \cite{tran2018spectral,xiang2021reverse,xiang2019benchmark,villarreal2020confoc} &
  \cite{yoshida2020disabling,weber2020rab,borgnia2021strong,li2021anti,jia2020certified,geiping2021doesn,hayase2021spectre} \\
& T$^F$ & & \cite{xiang2021reverse} &
  \cite{weber2020rab,li2021anti} \\
&  BL & \checkmark& &
\cite{geiping2021doesn,borgnia2021dp,li2021anti} \\
  \bottomrule
\end{tabular}%}
\end{table}
\begin{table}[h!]
\centering
\caption{Matching poisoning test time attack strategies and defenses applied after training. For each defense, we denote on which type of attack strategies the defense was evaluated. We omit indiscriminate attacks, as there are no corresponding defenses at test time (yet). }\label{table:testDefenses}
%\resizebox{\textwidth}{!} {%
\begin{tabular}{lcm{2.1cm}>{\raggedright}m{2.35cm}>{\raggedright}m{2.5cm}m{2.5cm}}
\toprule
\multicolumn{2}{c}{Attack}  & \multicolumn{4}{c}{Defenses} \\
\cmidrule(r){1-2}\cmidrule(r){3-6}
 & Strategy  &
 Model \newline  inspection &
  Trigger \newline  reconstruction &
  Model \newline  sanitization &
 Test data \newline  sanitization \\
 \midrule
Targeted &  - & \cite{zhu2021clear} & & \cite{zhu2021clear} & \\ \addlinespace 
\multirow{3}{*}{Backdoor}&
  T$^P$ &
  \cite{tang2019demon,chen2018detecting,kolouri2020universal,zhang2021tad,shen2021backdoor,chen2019deepinspect,Xu2021MetaAudio,bajcsy2021baseline,xiang2021red,soremekun2020exposing} &
  \cite{guo2019tabor,wangneural,liu2019abs,udeshi2019model,qiao2019defending,cheng2020defending,dong2021black,xiang2021reverse} &
  \cite{liu2018fine,zeng2020deepsweep,yoshida2020disabling,li2021neural,zhao2020bridging,qiao2019defending,chen2019deepinspect,zhu2020gangsweep,wu2021adversarial} &
  \cite{doan2020februus,li2020rethinking,zeng2020deepsweep,veldanda2020nnoculation,wangneural,chou2018sentinet,gao2019strip,sarkar2020backdoor,qi2020onion,villarreal2020confoc} \\
  
  %\addlinespace
& T$^F$ &
  \cite{tang2019demon,shen2021backdoor,huang2019neuroninspect,Xu2021MetaAudio,soremekun2020exposing} &
  \cite{xiang2020detection,zhu2020gangsweep,liu2019abs,xiang2021red} &
  \cite{zhu2020gangsweep, zeng2020deepsweep,li2021neural,wu2021adversarial} &
  \cite{zeng2020deepsweep} \\
  
  %\addlinespace
& T$^S$ & & & \cite{DBLP:conf/iccd/LiuXS17} &
  \cite{DBLP:conf/iccd/LiuXS17} \\
  %\addlinespace

  \bottomrule
\end{tabular}%}
\end{table}


\begin{table}[t]
\centering
\caption{Matching poisoning attack strategies and defenses. For each defense, we depict on which attack strategy (as defined in Section~\ref{sec::attacks}) the defense was evaluated. We omit strategies in the table that were not mitigated yet, including bilevel backdoors, and clean label bilevel indiscriminate poisoning. We mark cells with \dashmark\xspace if the corresponding defense category have not been investigated so far for the corresponding attack. Conversely, we mark cells with \xmark\xspace if corresponding defense has no sense and cannot be applied.}
\label{tab:my-table}
  \renewcommand{\arraystretch}{.9}
\setlength\tabcolsep{1pt} \begin{tabular}{@{}ccc|ccccc|c@{}}
\toprule
\multicolumn{3}{c}{\multirow{2}{*}{Attack}} & \multicolumn{6}{c}{Defenses} \\
\multicolumn{3}{c}{} & \multicolumn{5}{c}{Training time} & Test time \\ \midrule
 & Strategy & \begin{tabular}[c]{@{}c@{}}Clean\\ label\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training data\\ sanitization\end{tabular} & \begin{tabular}[c]{@{}c@{}}Robust \\ training\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ inspection\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ sanitization\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trigger\\ reconstruction\end{tabular} & \begin{tabular}[c]{@{}c@{}}Test data\\ sanitization\end{tabular} \\ \midrule
\multirow{2}{*}{\rotvertical{Indiscriminate}} & LF &  & \cite{paudice2018label, DBLP:journals/corr/LaishramP16,taheri2020defending} & \begin{tabular}[c]{@{}c@{}}\cite{hong2020effectiveness,levine2020deep,biggio11labelnoise}\\ \cite{DBLP:conf/itasec/DemontisBFGR17,rosenfeld2020certified}\end{tabular} & \dashmark & \dashmark & \xmark & \xmark  \\
\addlinespace\addlinespace\addlinespace\addlinespace\addlinespace\addlinespace
 & BL &  & \cite{frederickson2018attack,2017arXiv170603691S} & \cite{nelson2009misleading,biggio2011bagging, jia2020certified, private_learners_ma_2019} & \dashmark & \dashmark & \xmark & \xmark \\\addlinespace\midrule
\addlinespace
\multirow{3}{*}{\rotvertical{Targeted}} & BL &  & \cite{frederickson2018attack,hayase2021spectre} &  &  &  & \xmark & \xmark \\
 & BL & \checkmark &  & \cite{geiping2021doesn,borgnia2021dp,borgnia2021strong} &  &  &  \xmark&  \xmark\\
 & FC & \checkmark & \cite{peri2020deep} & \cite{geiping2021doesn,borgnia2021dp,li2021anti,hong2020effectiveness} & \cite{zhu2021clear} & \cite{zhu2021clear} &  &  \\
 \addlinespace \midrule
 \addlinespace
\multirow{5}{*}{\rotvertical{Backdoor}}  & BL & \checkmark & \dashmark & \cite{geiping2021doesn,borgnia2021dp,li2021anti} & \dashmark & \dashmark & \dashmark &  \xmark\\
& T$^P$ &  & \begin{tabular}[c]{@{}c@{}}\cite{tran2018spectral,villarreal2020confoc}\\ \cite{xiang2019benchmark,xiang2021reverse}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\cite{yoshida2020disabling,weber2020rab,borgnia2021strong}\\ \cite{li2021anti,jia2020certified,geiping2021doesn}\\ \cite{hayase2021spectre}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\cite{tang2019demon,chen2018detecting,kolouri2020universal}\\ \cite{zhang2021tad,shen2021backdoor,chen2019deepinspect,Xu2021MetaAudio}\\ \cite{bajcsy2021baseline,xiang2021red,soremekun2020exposing}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\cite{liu2018fine,zeng2020deepsweep,yoshida2020disabling}\\ \cite{zhao2020bridging,qiao2019defending,chen2019deepinspect}\\ \cite{li2021neural,zhu2020gangsweep,wu2021adversarial}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\cite{guo2019tabor,wangneural,liu2019abs}\\ \cite{udeshi2019model,qiao2019defending,cheng2020defending}\\ \cite{dong2021black,xiang2021reverse}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\cite{doan2020februus,li2020rethinking,zeng2020deepsweep,veldanda2020nnoculation}\\ \cite{wangneural,chou2018sentinet,gao2019strip,sarkar2020backdoor}\\ \cite{qi2020onion,villarreal2020confoc}\end{tabular} \\\addlinespace
 & T$^F$ &  & \cite{xiang2021reverse} & \cite{weber2020rab,li2021anti} & \begin{tabular}[c]{@{}c@{}}\cite{tang2019demon,shen2021backdoor,huang2019neuroninspect}\\ \cite{Xu2021MetaAudio,soremekun2020exposing}\end{tabular} & \cite{zhu2020gangsweep, zeng2020deepsweep,li2021neural,wu2021adversarial} & \begin{tabular}[c]{@{}c@{}}\cite{xiang2020detection,zhu2020gangsweep}\\ \cite{liu2019abs,xiang2021red}\end{tabular} & \cite{zeng2020deepsweep} \\\addlinespace
 & T$^S$ &  &  &  &  & \cite{DBLP:conf/iccd/LiuXS17} &  & \cite{DBLP:conf/iccd/LiuXS17} \\
 \bottomrule
\end{tabular}%
%}
\end{table}
\end{comment}


\begin{comment}
\begin{table}[t]
\centering
\caption{Matching poisoning attack strategies and defenses. \textcolor{red}{Training- and test-time defenses consider respectively the training and test time strategy of attacks in Table~\ref{table:poisoning_categorization}.} For each defense, we depict on which attack strategy (as defined in Section~\ref{sec::attacks}) the defense was evaluated. We omit strategies in the table that were not mitigated yet, including bilevel backdoors, and clean label bilevel indiscriminate poisoning. We mark cells with \dashmark\xspace if the corresponding defense category have not been investigated so far for the corresponding attack. Conversely, we mark cells with \xmark\xspace if corresponding defense has no sense and cannot be applied.}
\label{table:matching_attack_defenses}
\setlength\tabcolsep{3.1pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}P{0.1cm}P{0.25cm}P{0.25cm}P{0.7cm}|P{1.8cm}P{2.4cm}P{1.8cm}P{1.8cm}P{1.9cm}|P{1.7cm}@{}}
\toprule
\multicolumn{4}{c}{\multirow{2}{*}{Attack}} & \multicolumn{6}{c}{Defenses} \\
\multicolumn{4}{c}{} & \multicolumn{5}{c}{Training time} & Test time \\ \midrule
 & $\vct \delta$ & $\vct t$ & \begin{tabular}[c]{@{}c@{}}Clean\\ label\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training data\\ sanitization\end{tabular} & \begin{tabular}[c]{@{}c@{}}Robust \\ training\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ inspection\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ sanitization\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trigger\\ reconstruction\end{tabular} & \begin{tabular}[c]{@{}c@{}}Test data\\ sanitization\end{tabular} \\ \midrule
\multirow{3}{*}{\rotvertical{Indiscr.}} & LF & - &  & \cite{paudice2018label, DBLP:journals/corr/LaishramP16,taheri2020defending} & \cite{hong2020effectiveness,levine2020deep,biggio11labelnoise,DBLP:conf/itasec/DemontisBFGR17,rosenfeld2020certified} & \dashmark & \dashmark & \xmark & \xmark \\
 & BL & - &  & \cite{frederickson2018attack,2017arXiv170603691S} & \cite{nelson2009misleading,biggio2011bagging, jia2020certified, private_learners_ma_2019} & \dashmark & \dashmark & \xmark & \xmark \\
 & BL & - & \checkmark & \dashmark & \dashmark & \dashmark & \dashmark & \xmark & \xmark \\ \midrule
\multirow{3}{*}{\rotvertical{Targeted}} & BL & - &  & \cite{frederickson2018attack,hayase2021spectre} & \dashmark & \dashmark & \dashmark & \xmark & \textcolor{red}{\dashmark} \\
 & FC & - & \checkmark & \cite{peri2020deep} & \cite{geiping2021doesn,borgnia2021dp,li2021anti,hong2020effectiveness} & \cite{zhu2021clear} & \cite{zhu2021clear} & \xmark & \textcolor{red}{\dashmark} \\
 & BL & - & \checkmark & \dashmark & \cite{geiping2021doesn,borgnia2021dp,borgnia2021strong} & \dashmark & \dashmark & \xmark & \\ \midrule
\multicolumn{1}{l}{\multirow{7}{*}{\rotvertical{Backdoor}}} & T$^P$ & T$^P$ &  & \cite{tran2018spectral,xiang2021reverse,xiang2019benchmark,villarreal2020confoc} & \cite{yoshida2020disabling,weber2020rab,borgnia2021strong,li2021anti,jia2020certified,geiping2021doesn,hayase2021spectre} & \cite{tang2019demon,chen2018detecting,kolouri2020universal,zhang2021tad,shen2021backdoor,chen2019deepinspect,Xu2021MetaAudio,bajcsy2021baseline,xiang2021red,soremekun2020exposing} & \cite{liu2018fine,zeng2020deepsweep,yoshida2020disabling,zhao2020bridging,qiao2019defending,chen2019deepinspect,li2021neural,zhu2020gangsweep,wu2021adversarial} & \cite{guo2019tabor,wangneural,liu2019abs,udeshi2019model,qiao2019defending,cheng2020defending,dong2021black,xiang2021reverse} & \cite{doan2020februus,li2020rethinking,zeng2020deepsweep,veldanda2020nnoculation,wangneural,chou2018sentinet,gao2019strip,sarkar2020backdoor,qi2020onion,villarreal2020confoc} \\
\multicolumn{1}{l}{} & T$^S$ & T$^S$ &  & \dashmark & \dashmark & \dashmark & \cite{DBLP:conf/iccd/LiuXS17} & \dashmark & \cite{DBLP:conf/iccd/LiuXS17} \\
\multicolumn{1}{l}{} & T$^F$ & T$^F$ &  & \cite{xiang2021reverse} & \cite{weber2020rab,li2021anti} & \cite{tang2019demon,shen2021backdoor,huang2019neuroninspect,Xu2021MetaAudio,soremekun2020exposing} & \cite{zhu2020gangsweep, zeng2020deepsweep,li2021neural,wu2021adversarial} & \cite{xiang2020detection,zhu2020gangsweep,liu2019abs,xiang2021red} & \cite{zeng2020deepsweep} \\ 
& BL & T$^P$ & \checkmark & \dashmark & \cite{geiping2021doesn,borgnia2021dp,li2021anti} & \dashmark & \dashmark & \dashmark & \dashmark \\
\multicolumn{1}{l}{} & FC & T$^P$ & \checkmark & \dashmark & \dashmark & \dashmark & \dashmark & \dashmark & \dashmark \\
\multicolumn{1}{l}{} & BL & T$^F$ &  & \dashmark & \dashmark & \dashmark & \dashmark & \dashmark & \dashmark \\
\bottomrule
\end{tabular}
\end{table}
\end{comment}


\begin{table}[t]
\centering
\caption{Matching poisoning attack strategies and defenses. For each defense, we depict on which attack strategy (as defined in Section~\ref{sec::attacks}) the defense was evaluated. We mark cells with \dashmark\xspace if the corresponding defense category have not been investigated so far for the corresponding attack. Conversely, we mark cells with \xmark\xspace if corresponding defense has no sense and cannot be applied.}
\label{table:matching_attack_defenses}
\setlength\tabcolsep{3.1pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}P{0.1cm}P{0.25cm}P{0.25cm}P{0.7cm}|P{1.8cm}P{2.4cm}|P{1.8cm}P{1.8cm}P{1.9cm}P{1.7cm}@{}}
\toprule
\multicolumn{4}{c}{\multirow{2}{*}{Attack}} & \multicolumn{6}{c}{Defenses} \\
\multicolumn{4}{c}{} & \multicolumn{5}{c}{Training Time} & Test Time \\ \midrule
 & $\vct \delta$ & $\vct t$ & \begin{tabular}[c]{@{}c@{}}Clean\\ Label\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training Data\\ Sanitization\end{tabular} & \begin{tabular}[c]{@{}c@{}}Robust \\ Training\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ Inspection\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ Sanitization\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trigger\\ Reconstruction\end{tabular} & \begin{tabular}[c]{@{}c@{}}Test Data\\ Sanitization\end{tabular} \\ \midrule
\multirow{3}{*}{\rotvertical{Indiscr.}} & LF & - &  & \cite{paudice2018label, DBLP:journals/corr/LaishramP16,taheri2020defending} & \cite{hong2020effectiveness,levine2020deep,biggio11labelnoise,DBLP:conf/itasec/DemontisBFGR17,rosenfeld2020certified} & \dashmark & \dashmark & \xmark & \xmark \\
 & BL & - &  & \cite{frederickson2018attack,2017arXiv170603691S} & \cite{nelson2009misleading,biggio2011bagging, jia2020certified, private_learners_ma_2019} & \dashmark & \dashmark & \xmark & \xmark \\
 & BL & - & \checkmark & \dashmark & \dashmark & \dashmark & \dashmark & \xmark & \xmark \\ \midrule
\multirow{3}{*}{\rotvertical{Targeted}} & BL & - &  & \cite{frederickson2018attack} & \dashmark & \dashmark & \dashmark & \xmark & \textcolor{red}{\dashmark} \\
 & FC & - & \checkmark & \cite{peri2020deep} & \cite{geiping2021doesn,borgnia2021dp,li2021anti,hong2020effectiveness} & \textcolor{red}{\cite{zhu2021clear,tang2019demon}} & \cite{zhu2021clear} & \xmark & \textcolor{red}{\dashmark} \\
 & BL & - & \checkmark & \dashmark & \cite{geiping2021doesn,borgnia2021dp,borgnia2021strong} & \dashmark & \dashmark & \xmark & \textcolor{red}{\dashmark} \\ \midrule
\multicolumn{1}{l}{\multirow{7}{*}{\rotvertical{Backdoor}}} & T$^P$ & T$^P$ &  & \textcolor{red}{\cite{tran2018spectral,xiang2021reverse,xiang2019benchmark,villarreal2020confoc,hayase2021spectre}} & \textcolor{red}{\cite{yoshida2020disabling,weber2020rab,borgnia2021strong,li2021anti,jia2020certified,geiping2021doesn}} & \cite{tang2019demon,chen2018detecting,kolouri2020universal,zhang2021tad,shen2021backdoor,chen2019deepinspect,Xu2021MetaAudio,bajcsy2021baseline,xiang2021red,soremekun2020exposing} & \cite{liu2018fine,zeng2020deepsweep,yoshida2020disabling,zhao2020bridging,qiao2019defending,chen2019deepinspect,li2021neural,zhu2020gangsweep,wu2021adversarial} & \cite{guo2019tabor,wangneural,liu2019abs,udeshi2019model,qiao2019defending,cheng2020defending,dong2021black,xiang2021reverse} & \cite{doan2020februus,li2020rethinking,zeng2020deepsweep,veldanda2020nnoculation,wangneural,chou2018sentinet,gao2019strip,sarkar2020backdoor,qi2020onion,villarreal2020confoc} \\
\multicolumn{1}{l}{} & T$^S$ & T$^S$ &  & \dashmark & \dashmark & \textcolor{red}{\cite{shen2021backdoor}} & \textcolor{red}{\cite{DBLP:conf/iccd/LiuXS17,liu2018fine,zeng2020deepsweep}} & \dashmark& \textcolor{red}{\cite{DBLP:conf/iccd/LiuXS17,veldanda2020nnoculation}}\\
\multicolumn{1}{l}{} & T$^F$ & T$^F$ &  & \textcolor{red}{\cite{xiang2021reverse,hayase2021spectre}} & \cite{weber2020rab,li2021anti} & \textcolor{red}{\cite{tang2019demon,shen2021backdoor,huang2019neuroninspect,Xu2021MetaAudio,soremekun2020exposing,xiang2021red}} & \cite{zhu2020gangsweep, zeng2020deepsweep,li2021neural,wu2021adversarial} & \textcolor{red}{\cite{xiang2020detection,zhu2020gangsweep,liu2019abs,xiang2021red,xiang2021reverse}} & \textcolor{red}{\cite{zeng2020deepsweep,gao2019strip}} \\ 
\multicolumn{1}{l}{} & FC & T$^P$ & \checkmark & \textcolor{red}{\cite{hayase2021spectre}} & \textcolor{red}{\cite{geiping2021doesn,borgnia2021dp,li2021anti}} & \textcolor{red}{\cite{zhu2021clear}} & \textcolor{red}{\cite{zhu2021clear,zhu2020gangsweep,li2021neural,wu2021adversarial}} & \dashmark & \textcolor{red}{\cite{li2020rethinking}} \\
\multicolumn{1}{l}{} & BL & T$^F$ &  & \dashmark & \dashmark & \textcolor{red}{\cite{shen2021backdoor}} & \textcolor{red}{\cite{wu2021adversarial}} & \textcolor{red}{\cite{zhu2020gangsweep}} & \textcolor{red}{\cite{zeng2020deepsweep}} \\
& BL & T$^P$ & \checkmark & \dashmark & \dashmark & \dashmark & \dashmark & \dashmark & \dashmark \\
\bottomrule
\end{tabular}
\end{table}
